Membership Privacy Protection for Image Translation Models via Adversarial Knowledge Distillation

Image-to-image translation models are shown to be vulnerable to the Membership Inference Attack (MIA), in which the adversary's goal is to identify whether a sample is used to train the model or not. With daily increasing applications based on image-to-image translation models, it is crucial to protect the privacy of these models against MIAs. We propose adversarial knowledge distillation (AKD) as a defense method against MIAs for image-to-image translation models. The proposed method protects the privacy of the training samples by improving the generalizability of the model. We conduct experiments on the image-to-image translation models and show that AKD achieves the state-of-the-art utility-privacy tradeoff by reducing the attack performance up to 38.9% compared with the regular training model at the cost of a slight drop in the quality of the generated output images. The experimental results also indicate that the models trained by AKD generalize better than the regular training models. Furthermore, compared with existing defense methods, the results show that at the same privacy protection level, image translation models trained by AKD generate outputs with higher quality; while at the same quality of outputs, AKD enhances the privacy protection over 30%.

==> Sections/01_intro.tex <==
\section{Introduction}
\label{sec:intro}
The recent advances in the field of Artificial Intelligence (AI) have lead to the creation of new applications in computer vision, natural language processing, signal processing, etc. Among these applications, image-to-image translation (image translation in short) models have gained increasing attention. Image translation models map images from one domain to an image in another domain. Some examples for the tasks that image translation models are used for including but not limited to  data synthesis (dataset augmentation), image colorization, and pose transfer~\cite{pix2pix}. The mentioned examples are based on Conditional Generative Adversarial Network (cGAN)~\cite{pix2pix,pix2pixHD} which is commonly used in supervised image translation models.
%for mapping one image that is given as a condition to the model to the output image.

Deep models may leak information about the datasets or the model, even with black-box access to the model. Therefore, as the practical usage of the image translation models increases, including models trained with sensitive data such as medical dataset, the privacy concerns related to these model raises.

Membership Inference Attacks (MIA) is a way to evaluate the leakage of a model where adversary ties to find out whether a given sample is used in training of the target model or not. It is recently shown in~\cite{ICCV'21} that the supervised image translation models, which are the focus of this paper, are vulnerable to MIA, and the adversary can predict the membership status of the samples with a high accuracy. Membership status is considered as personal data~\cite{law}, so it should be kept private. However,  image to image translation models are highly susceptible to leak membership status of the data samples. Authors in~\cite{ICCV'21} also show that the applying number of widely used defenses for improving the privacy of deep learning models either did not either improve the privacy of the models or generate high quality images. 

In this paper, we aim to propose a defense method against MIA which compared to the existing defenses achieves a better utility-privacy trade-off for image translation models. 
In other words, at the same privacy level, the proposed defense based on Adversarial Knowledge Distillation (AKD) generates higher quality images compared to other defenses. 
%In other words, at the same privacy level, the proposed defense based on Adversarial Knowledge Distillation (AKD) generates higher quality images compared to other defenses. 
AKD combines the adversarial training~\cite{GAN} with knowledge distillation mechanism~\cite{hinton2015distilling}. In details, the private model is initially trained with the private dataset. Then, the private model is used as a teacher model to train a student model in an adversarial manner using a proxy dataset. The proxy dataset is a set of unlabelled input images for which the teacher model generates the label. Finally, the student model is deployed as a public model to prevent the leakage of the private model. 
% In the proposed method, the private model is initially trained with the private dataset then used as a teacher model to distill knowledge to a student model in an adversarial manner using a proxy dataset.
% The proxy dataset is a set of unlabelled input images for which the teacher model generates the label. 
%In addition, triplet loss is used as a regularizer in the distillation process that helps to further mitigate MIA by forcing a margin between the generated samples and samples from a real dataset.

Although knowledge distillation is used as a defense method against MIA in the earlier work, Distillation for Membership Privacy (DMP)~\cite{DMP}, the proposed knowledge-distillation based defense method in this paper is different from DMP in multiple aspects. First, the proposed method uses a adversarial distillation method including a discriminator in the training that helps the generator to create images with higher quality. The other difference is that DMP is proposed for image classification models, and the unlabelled data is sampled before distillation using the entropy of the logits at the model output. However, such approach is not applicable to the image-to-image translation models. In our method, no pre-processing is needed to be applied to the unlabelled data.

Membership leakage~\cite{monte_carlo,overfitting} is closely related to overfitting of the model to the training data (i.e., the generalization error). In addition, overfitting causes dataset memorization which is a key challenge in training generative models (including the image-to-image translation models)~\cite{gan-limited-1,gan-limited-2}. Therefore the reduction of overfitting helps improving the privacy of the model as well as avoiding the model to memorize data directly from the observed samples during the training. We show that qualitatively and quantitatively that the adversarial knowledge distillation method reduces overfitting by reducing the generalization gap of image to image translation models.

The contribution of the proposed method are summarized as:
\begin{itemize}
  \item We propose a novel method of knowledge distillation for image translation models which is used as a defense method against MIA. To best of our knowledge, our proposed method is the first defense method on image translation models that achieves membership privacy while generating realistic outputs similar to the models trained with no constraints on privacy. The proposed defense method is also a post-hoc method, meaning that it can applied to models that have already been trained.
  %\item \saeed{Use of triplet loss is proposed a regularization method that reduces the membership inference attack}
  \item We show that the proposed method reduces the overfitting which improves privacy and reduces the data replication in the trained generative models.  
  \item Through extensive experiments we show the that AKD achieves state-of-the-art tradeoff between the quality of the generated samples and the membership privacy for image translation models. 
\end{itemize}

The remainder of the paper is organized as follows: Preliminaries are discussed in Section~\ref{sec:prem}. The proposed method is introduced in Section~\ref{sec:proposed}. The experimental setup is discussed in Section~\ref{sec:exp_setup} followed by the experiments in Section~\ref{sec:exp}. Section~\ref{sec:related_work} briefly reviews the related works, and Section~\ref{sec:conc} concludes the paper.  


%todo: 
%mention LOGAN

